SWIM: Vision-Language-Grounded Soft Whole-Body Interactive Manipulation

Soft and continuum robots enable manipulation through distributed body deformation and contact, yet translating language and visual context into executable whole-body actuation remains a fundamental challenge. We present SWIM, a framework that maps an initial RGB observation and a language instruction to a complete actuation-command sequence. Its vision-language-action (VLA) policy, SWIM-VLA, combines a diffusion action head with Visual Soft Proprioception (VSP) through a shared representation of RGB observations, language instructions, and tendon states. The diffusion head models conditional distributions of expert command chunks, while VSP supervises ordered body-anchor predictions using simulation ground truth, encouraging the representation to retain body geometry when learning from limited demonstrations. Embodied mechanical intelligence supports physical execution of command sequences generated through iterative virtual rollout from evolving simulated observations, with intrinsic compliance providing local contact adaptation without online policy queries. We evaluate SWIM on packing, reaching, and grasping on a planar tendon-driven soft robot, with grasping targets anchored. In simulation, SWIM-VLA achieves success rates of 100\%, 96\%, and 88\%, respectively, outperforming an adapted OpenVLA-OFT baseline and controlled ablations. On hardware, SWIM achieves success rates of 100\%, 80\%, and 75\%, compared with 75\%, 40\%, and 25\% for direct online deployment of the same policy checkpoint.

==> Tex/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% 



% \Ke{Soft and continuum robots distribute deformation and compliance along their bodies, enabling object manipulation through contacts formed along the deformable body rather than exclusively at an end effector~\cite{rus2015design,walker2013continuous,graule2022contact}.}

Soft and continuum robots distribute deformation and compliance along their
bodies, enabling object manipulation through contacts formed along the
deformable body rather than exclusively at an end effector
~\cite{rus2015design,walker2013continuous,graule2022contact}. Their bodies therefore serve simultaneously as the kinematic
structure that generates motion and the contact interface
that interacts with objects and the environment
~\cite{calisti2011octopus}.
This distributed interaction expands the range of achievable
wrapping, enveloping, and contact-rich manipulation
behaviors~\cite{li2016progressive}, but also couples whole-body
configuration, motion, and contact throughout task
execution~\cite{dellasantina2020dynamic}.
Prior work on this capability has developed along two
complementary directions: regulating whole-body shape
and configuration~\cite{almanzor2023staticshape}, and coordinating
body motion and distributed contact for
manipulation~\cite{graule2022contact}.

For configuration control, Pustina et al. designed feedback laws to regulate prescribed soft-robot shapes under model uncertainty and constant disturbances~\cite{pustina2023shape}, while Almanzor et al. used deep visual inverse kinematics to reach user-specified full-body target shapes~\cite{almanzor2023staticshape}. Beyond configuration control, early OctArm experiments demonstrated teleoperated whole-arm grasping and object handling~\cite{mcmahan2006field}. Marchese et al. planned motions of an entirely soft arm while accounting for its changing body envelope in confined environments ~\cite{marchese2014wholearm}. Li and Xiao planned probing and progressive contact formation for whole-arm grasping in clutter ~\cite{li2016progressive}. More recent work incorporated distributed tactile sensing and hierarchical control for autonomous underwater grasping ~\cite{deldottore2026peripheral}, while Yang et al. learned whole-body grasping from actuation-space demonstrations ~\cite{yang2026lightweight}. Across these systems, however, the task class and interaction structure are fixed before deployment. Shape controllers receive prescribed configurations~\cite{pustina2023shape,almanzor2023staticshape}; motion and contact planners optimize user-specified paths or predefined grasp objectives~\cite{marchese2014wholearm,li2016progressive}; and autonomous or learned systems remain organized around a fixed grasping behavior encoded by a control hierarchy or skill-specific demonstrations~\cite{deldottore2026peripheral,yang2026lightweight}. \textcolor{blue}{These formulations address control or grasp synthesis after
the desired configuration, objective, or skill has been
specified, but do not directly resolve the task-grounding
problem considered here.
In a more general task setting, the robot must infer the
requested whole-body behavior and task-relevant target from
language and the observed scene, rather than receive a
prescribed configuration or a skill-specific control
objective.
This requires a unified interface that connects semantic
intent and visual context to physically executable
whole-body actuation.}
% Consequently, reported generalization is primarily intra-skill, covering variations in target pose, object geometry, or contact conditions within the same predefined behavior \cite{deldottore2026peripheral,yang2026lightweight}. More general task-level manipulation requires a robot to interpret
% semantically specified goals, identify task-relevant entities in the
% observed scene, and synthesize an appropriate whole-body deformation and
% contact strategy. Meeting these demands calls for an interface that connects
% semantic intent and visual context to physically executable whole-body
% actuation.




Vision-language-action (VLA) models map language instructions and visual
observations to robot actions, but most established formulations target
rigid manipulators using Cartesian end-effector motions, gripper states, or
joint commands
\cite{zitkovich2023rt2,kim2024openvla,kim2025fine}.
Several recent VLA extensions to soft and continuum robots build on
established rigid-robot formulations while adapting their action interfaces
to deformable platforms. \textcolor{blue}{These studies focus on end-effector-centered object
manipulation \cite{su2025bridging,wei2026manisoft},
target tracking or navigation using discrete motor commands
\cite{ng2025endovla,lin2026bilivla}, or the generation of
predefined motion types and robot-specific behavior families
through low-level actuation
\cite{tang2026tmrvla,liu2026wholebody}.}
% They either focus on end-effector-centered object manipulation
% \cite{su2025bridging,wei2026manisoft}, use discrete motor commands for
% target tracking or navigation
% \cite{ng2025endovla,lin2026bilivla}, or map predefined motion types and
% robot-specific behavior families to low-level actuation
% \cite{tang2026tmrvla,liu2026wholebody}.
% Three mismatches for
% soft whole-body manipulation.
\textcolor{blue}{Extending these advances to manipulation through distributed
body contact raises three coupled design challenges.}
First, at the action-interface level, end-effector commands constrain only distal motion and do not uniquely specify the whole-body manipulation required by the task instructions~\cite{graule2022contact}. 
\Ke{Second, soft robots introduce a whole-body state-representation
mismatch. Rigid-robot VLAs can often separate task-level action
generation from low-level configuration regulation through known
kinematics and an independent controller.\cite{kim2024openvla} For tendon-driven soft
robots, by contrast, the effect of an actuation command depends
on the current configuration~\cite{rao2021model}. Moreover,
low-dimensional tendon measurements do not fully characterize
the realized whole-body geometry under nonlinear deformation
and contact~\cite{rus2015design}. Consequently,
the state relevant to whole-body manipulation extends beyond
the tendon state alone.}
% Second, soft robots introduce a whole-body state-representation
% mismatch. Rigid-robot VLAs can often separate task-level action
% generation from low-level configuration regulation through known
% kinematics and an independent controller. For tendon-driven soft robots,
% by contrast, the effect of an actuation command depends on the current
% tendon state, requiring explicit state conditioning. Since tendon state does not uniquely determine the realized whole-body
% geometry under nonlinear deformation and contact
% \cite{rus2015design,almanzor2023staticshape,wang2025spirobs}, explicit
% geometric supervision is further needed to ensure that the visual
% representation preserves this information.

% Beyond the action interface, soft robots also face a whole-body state-representation mismatch: 
% actuation commands do not directly reveal the realized whole-body geometry because deformation is nonlinear and interaction-dependent~\cite{rus2015design,almanzor2023staticshape,wang2025spirobs}. Consequently, action-only supervision does not ensure that the policy encodes the realized whole-body geometry.
% \Ke{Third, at the execution level, VLA inference cost can
% limit the rate of closed-loop policy updates~\cite{kim2025fine}.
% Inference and communication latency, together with
% action-chunk scheduling, can delay command application
% relative to the observations used for prediction~\cite{black2025realtime}.
% For soft whole-body manipulation, such delays raise the risk
% of issuing commands that no longer match the evolving
% deformation and contact state.}
Together, these mismatches call for a vision-language-grounded framework for soft whole-body manipulation that translates task specifications into executable actuation commands, explicitly represents the evolving whole-body shape, and leverages mechanical intelligence during execution, rather than directly transferring conventional rigid-robot VLA formulations that rely on high-frequency closed-loop correction.
% We therefore study
% \emph{vision-language-grounded soft whole-body manipulation}: given an
% initial task-scene observation, a language instruction, and the robot's
% initial tendon state, how can a soft robot generate a physically executable
% actuation sequence whose success depends on distributed body deformation
% and contact rather than distal motion alone?

% Vision-language-action (VLA) models instantiate such an interface by mapping
% language instructions and visual observations to robot actions. Existing
% VLA systems have been developed for rigid manipulators, where actions are
% represented as Cartesian end-effector motions, gripper states, or joint
% commands \cite{zitkovich2023rt2,kim2024openvla,kim2025oft}. Recent work has begun to extend this paradigm to soft and continuum robots.
% Su et al.\ fine-tune OpenVLA-OFT and $\pi_0$ using Cartesian end-effector
% states and actions \cite{su2025bridging}; EndoVLA predicts discrete bending
% commands for visual target tracking \cite{ng2025endovla}; BiliVLA addresses stage-conditioned biliary navigation by jointly predicting discrete motor commands and a grounded target box\cite{lin2026bilivla}. And ManiSoft
% benchmarks vision-language policies using expert trajectories generated from
% task-specific end-effector waypoints \cite{wei2026manisoft}. Complementary
% work grounds semantic commands more directly into actuation. TMR-VLA maps
% visual observations and language-specified motion types to low-level actuation
% voltages \cite{tang2026tmrvla}, while Liu et al.\ map MLLM-generated semantic
% responses to tendon-actuation trajectories for expressive soft-trunk
% interaction \cite{liu2026wholebody}. Taken together, these formulations remain only partially aligned with soft
% whole-body manipulation, as they either induce soft-body behavior through
% end-effector or tracking objectives or organize it around predefined motion
% types and robot-specific motion families. On the perception--action side, a
% distal action does not specify the distributed deformation and contact
% required for execution, while conventional action supervision does not
% explicitly require the learned representation to preserve the robot's
% whole-body geometry. On the execution side, relying on repeated centralized
% observation--action updates for local interaction correction overlooks a
% defining property of soft robots: their compliant morphology can passively
% accommodate bounded geometric and contact variations during physical
% execution. These characteristics motivate a soft-robot-specific VLA that
% uses visual and language context to determine task-relevant whole-body
% deformation and contact, directly generates the corresponding native
% actuation sequence, and exploits physical compliance to reduce repeated
% real-world policy correction. We therefore study
% \emph{vision-language-grounded whole-body manipulation}: given an initial
% observation of a task scene, a semantic instruction, and the robot's initial
% tendon state, how can a soft robot generate a physically executable
% actuation sequence whose success depends on distributed body deformation
% and contact rather than distal motion alone?

% Across these approaches, body behavior is
% either induced through end-effector or tracking objectives, or organized
% around predefined motion types and robot-specific motion families.
% Taken together, prior soft-robot whole-body methods and recent VLA/MLLM
% approaches leave open the problem of \emph{vision-language-grounded
% whole-body manipulation}: given an initial observation of a task scene and a semantic
% instruction, how can a soft robot synthesize a physically executable
% actuation sequence whose success depends on distributed body deformation
% and contact rather than distal motion alone?

% Taken together, existing soft-robot whole-body methods and VLA/MLLM approaches
% leave open the problem of \emph{vision-language-grounded whole-body
% manipulation}, in which a policy jointly determines, from the task instruction
% and visual scene, how the robot should use its body and which actions to
% execute.

% To address this gap, we introduce \methodname{}
% (\textbf{S}oft \textbf{W}hole-body \textbf{I}nteraction and
% \textbf{M}anipulation VLA), a body-aware, actuation-space VLA policy for
% soft-robot whole-body manipulation. Our contributions are:

\begin{figure*}[t]
   \centering
\includegraphics[page=6,width=170mm,trim=10mm 40mm 2mm 7mm,clip]{fig_new/framework_intro_v5.pdf}
   \caption{Motivation and design principles of SWIM for soft whole-body manipulation.}
   \label{fig:intro}
\end{figure*}

To address these mismatches, we introduce SWIM, a framework for
vision-language-grounded soft whole-body manipulation. Our contributions are:

\begin{itemize}
    \item \textbf{SWIM: a vision-language-grounded framework for soft whole-body
    interactive manipulation.}
    \textcolor{blue}{We introduce a framework that converts an initial
vision-language task specification into a complete
actuation-command sequence through iterative virtual
rollout conditioned on evolving simulated observations,
and executes the resulting sequence on a physical soft robot.}
%     We introduce a framework that converts an initial visual-language
% task specification into a complete actuation-command sequence
% through virtual rollout and executes it on a physical soft robot.

   \item \textbf{\methodname{}: a soft whole-body manipulation VLA.}
Within SWIM, we introduce SWIM-VLA, which conditions action
generation on the current tendon state and combines a command-space
diffusion action head for temporally coordinated command generation
with Visual Soft Proprioception (VSP). VSP uses ordered body-anchor
supervision to structure the shared representation around the robot's
realized whole-body geometry.
    % Within SWIM, \methodname{} addresses the action and representation
    % mismatches through an actuation-space diffusion action head and Visual
    % Soft Proprioception. The action head generates temporally coordinated
    % native commands, while VSP encourages the shared representation to encode
    % distributed body geometry.

    \item \textbf{Systematic simulation and physical validation.}
    We evaluate SWIM and \methodname{} on diverse non-contact and
    contact-rich whole-body tasks, perform controlled ablations of the diffusion action head and VSP, and validate command-sequence
    execution in simulation and on the physical robot.
\end{itemize}



% Together, the soft-robot whole-body literature and the VLA literature expose a missing connection between semantic task grounding and whole-body execution. Bridging this gap is nontrivial because similar end-effector states can correspond to substantially different whole-body configurations, obstacle clearances, contact patterns, and task outcomes. Moreover, on physical hardware, the current whole-body configuration is not directly available from practical sensing, while explicit reconstruction often requires additional sensors or dedicated estimation. What remains missing is a framework that grounds language and visual scene context into actions while maintaining awareness and coordination of the robot's whole-body configuration using deployable sensing.



% To address this gap, we formulate vision-language-grounded whole-body manipulation for soft robots, where language specifies the task and vision provides the scene context for coordinating the robot’s entire body. We introduce \methodname{} (Soft Whole-body Interaction and Manipulation VLA), a VLA policy that maps RGB observations and language instructions, together with tendon-length feedback readily available from the physical robot, to short-horizon actuation commands. By predicting commands directly in actuation space, \methodname{} avoids a hand-designed conversion from end-effector motion to tendon commands and enables direct coordination of whole-body motion. To make action prediction aware of the robot’s current whole-body configuration, we further propose Visual Soft Proprioception (VSP), a training-only auxiliary objective that predicts body-anchor locations from visual features. This supervision encourages the visual representation to encode the whole-body configuration without requiring body-anchor measurements or explicit shape reconstruction at deployment. We evaluate \methodname{} in simulation and on a physical soft robot across non-contact whole-body tasks and contact-rich manipulation tasks.

% The contributions of this paper are summarized as follows:
%



